Calibrated Reasoning: An Explanatory Verifier for Dynamic and Efficient Problem-Solving

Advanced test-time computing strategies are essential for scaling reasoning models, but their effectiveness is capped by the models' poor self-evaluation. We propose a pairwise Explanatory Verifier, trained via reinforcement learning (GRPO), that produces calibrated confidence scores and associated natural language reasoning for generated solutions. Our verifier improves the accuracy and efficiency of test-time strategies like best-of-n and self-reflection. Crucially, it excels at identifying challenging failure modes, such as when both candidate solutions are identically incorrect, succeeding where standard methods like majority voting fail.

==> 2.modelTraining.tex <==


\section{RL training of pairwise verifier}
\label{sec:verifier}

\ignore{
\begin{itemize}
    \item Problem formulation in equations
    \item Data curation for verifier training
    \item Stages of training -- context length, dataset sampling, ...
    \item Implementation details and hyperparams
    \item Analysis of behavior shifts from RL training (goes into results)
\end{itemize}
}

\textbf{Task description.} Given a question and two responses, the verifier is tasked with scoring both the responses in the range of [0,10], 0 being incorrect and 10 being correct. We chose the pairwise verifier based on the results shown by~\cite{deepseekverifier}.

\textbf{Training data.} We trained the verifier on a compact dataset consisting of 600 questions, \ignore{significantly less than the amount used in other works (18k in CTRL, )} each with roughly six response combinations, for a total of 240 training steps. To focus on the most informative cases, we sampled only high-difficulty questions. Constructing this dataset from Numina-Math presented several challenges. Even when using the Skywork-filtered subset as ground truth, significant noise remained. To mitigate this, we applied additional filtering criteria—restricting to open-ended questions (rather than multiple-choice), requiring a single correct answer, and enforcing other consistency checks. We also experimented with using pass@k as a proxy for question difficulty, but found that it increased noise in the data. Balancing the trade-off between difficulty and noise was therefore a critical part of our dataset curation process.

\textbf{Reward shaping.} A key contribution of our work is a reward-shaping strategy that produces ratings on a scale of 0–10, reflecting verifier confidence in an answer being correct or incorrect. The reward is inspired by Binary Cross-Entropy loss:  
\[
R(p, y) =
\begin{cases}
-4.5, & \text{if } p \notin [0, 10] \\
y \cdot \log(\tilde{p}) + (1-y) \cdot \log(1-\tilde{p}), & \text{otherwise}
\end{cases}
\]
where \(\tilde{p} = 0.1 + \tfrac{p}{10} \cdot 0.8\) is the rescaled prediction,  
\(p \in [0,10]\) is the predicted score, and \(y \in \{0,1\}\) is the ground truth. 
 
